Interpretable (not just posthoc-explainable) heterogeneous survivor bias-corrected treatment effects for assignment of postdischarge interventions to prevent readmissions

We used survival analysis to quantify the impact of postdischarge evaluation and management (E/M) services in preventing hospital readmission or death. Our approach avoids a specific pitfall of applying machine learning to this problem, which is an inflated estimate of the effect of interventions, due to survivors bias -- where the magnitude of inflation may be conditional on heterogeneous confounders in the population. This bias arises simply because in order to receive an intervention after discharge, a person must not have been readmitted in the intervening period. After deriving an expression for this phantom effect, we controlled for this and other biases within an inherently interpretable Bayesian survival framework. We identified case management services as being the most impactful for reducing readmissions overall.

==> postdischarge-pratenddefaultcategory.tex <==


\begin{restatable}[Wait time distribution $\mid $ observed]{lemma}{prAtEndRestateii}\label{thm:prAtEndii}\label {lem:waitcond} Suppose as in Lemma~\ref {lem:correctedlike} that the waiting time after intervention at time $\tau $ is distributed according to the density $g_\tau (T-\tau ).$ If $\tau $ is distributed \begin {equation} \tau \sim h(\tau ), \end {equation} then, the wait time distribution for admissions \textbf {where no intervention is observed} is \begin {equation} f(T| T< \tau ) = f_\infty (T) \end {equation} and the wait time distribution \textbf {where the intervention is observed} is \begin {align} f(T| T\geq \tau ) &= \int _0^\infty g_\tau (T-\tau )\left ( 1-\displaystyle \int _0^\tau f_\infty (u) \dd u \right ) h(\tau )\dd \tau . \end {align}\end{restatable}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndii}By conditioning, \begin {align} f(T | T\leq \tau ) &= \int _0^\infty f(T | T\leq \tau , \tau )h(\tau ) \dd \tau \nonumber \\ &= \int _0^\infty f_\infty (T) h(\tau ) \dd \tau \nonumber \\ &= f_\infty (T).\label {eq:waitcond} \end {align} The argument for $f(T|T\geq \tau )$ is the same.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Eq.~\ref {eq:phantomprob} is found by substituting the expression in Remark~\ref {lem:null} into the expression for the wait time distribution where no intervention is observed in Lemma~\ref {lem:waitcond} and integrating over the limits $\tau \in [0, c].$\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndiv}\par Consider a test function $\phi (T)$. As in Eq.~\ref {eq:tauTconditioning} we decompose its expectation \begin {equation} \mathbb {E}(\phi (T) | \tau _1,\ldots ,\tau _N) = \sum _{i=1}^{N+1} \mathbb {E}\left (\phi (T) | T\in [\tau _{i-1}, \tau _i)\right )\Pr \left (T\in [\tau _{i-1}, \tau _i)\right ), \end {equation} where we define $\tau _0\equiv 0$ and $\tau _{N+1} \equiv +\infty $. Conditional on the $i-1$-st intervention having been applied, we have \begin {align} \mathbb {E}\left (\phi (T) | T\in [\tau _{i-1}, \tau _i)\right ) &= \bigints _{\tau _{i-1}}^\tau \frac {g_{\tau _1,\tau _2,\ldots ,\tau _{i-1},\infty }(T-\tau _{i-1})}{\displaystyle \int _{\tau _{i-1}}^{\tau _i} g_{\tau _1,\tau _2,\ldots ,\tau _{i-1},\infty }(u-\tau _{i-1}) \dd u} \phi (T) \dd T \label {eq:Tsim_complete} \end {align} \par \begin {align} \Pr \left (T\in [\tau _{i-1}, \tau _i)\right ) &= \Pr \left ( T<\tau _i | T\geq \tau _{i-1} \right ) \Pr \left (T\geq \tau _{i-1} \right )\nonumber \\ &=\int _{\tau _{k-1}}^{\tau _{k}} g_{\tau _1,\ldots ,\tau _{k-1},\infty }(T-\tau _{k})\dd T \nonumber \\ &\qquad \times \left (1- \displaystyle \int _{0}^{\tau _1} f_\infty (T) \dd T - \displaystyle \sum _{k=1}^{i}\int _{\tau _{k}}^{\tau _{k+1}} g_{\tau _1,\ldots ,\tau _{k},\infty }(T-\tau _{k})\dd T \right ) \label {eq:complete_like} \end {align} \par \par \end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[]\phantomsection\label{proof:prAtEndv}Consider the expectation of a test function $\phi $ applied to the wait time $T$. We construct this expectation by conditioning on $T$ relative to $\tau $ \begin {equation} \mathbb {E}(\phi (T) | \tau ) = \mathbb {E}(\phi (T) | \tau , T\geq \tau )\Pr (T\geq \tau | \tau ) + \mathbb {E}(\phi (T)| \tau , T<\tau )\Pr (T<\tau | \tau ), \label {eq:tauTconditioning} \end {equation} where the first term in Eq.~\ref {eq:tauTconditioning} is the contribution to the expectation when the intervention is successfully performed and the second term is the contribution when the intervention is not performed. The expectation of $\phi $, conditional on the event occurring before time $\tau $ is the expectation of the truncated distribution \begin {equation} \mathbb {E}(\phi (T)\vert \tau , T<\tau ) = \dfrac {\int _0^\tau \phi (T) f_\infty (T)\dd T}{\int _0^\tau f_\infty (T)\dd T}. \end {equation} The probability of the condition $T<\tau $ is \begin {equation} \Pr (T<\tau \vert \tau ) = \int _0^\tau f_\infty (T)\dd T, \end {equation} so \begin {equation} \mathbb {E}(\phi (T)\vert \tau , T<\tau ) \Pr (T<\tau \vert \tau ) = \int _0^\infty \phi (T) f_\infty (T)\dd T. \end {equation} In the case where $T\geq \tau ,$ we have by definition of $g,$ \begin {equation} \mathbb {E}(\phi (T)\vert \tau , T\geq \tau ) = \int _\tau ^\infty \phi (T)g_\tau (T-\tau ) \dd T, \end {equation} where the probability of the corresponding condition follows \par \begin {equation} \Pr (T\geq \tau \vert \tau ) = \int _\tau ^\infty f_\infty (T)\dd T. \end {equation} \par Substituting these Eqs. into Eq.~\ref {eq:tauTconditioning} yields \par \begin {align} \mathbb {E}(\phi (T) \vert \tau ) &= \int _0^\tau \phi (T)f_\infty (T) \dd T + \int _\tau ^\infty \phi (T) g_\tau (T-\tau )\int _\tau ^\infty f_\infty (u) \dd u \dd T \nonumber \\ &= \int _0^\infty \phi (T)\left [ (1-H(T-\tau )) f_\infty (T) + H(T-\tau ) g_\tau (T-\tau )\int _\tau ^\infty f_\infty (u)\dd u \right ] \dd T, \end {align} where $H$ is the unit step function.\end{proof}

